To Aggregate or Not? Learning with Separate Noisy Labels

The rawly collected training data often comes with separate noisy labels collected from multiple imperfect annotators (e.g., via crowdsourcing). A typical way of using these separate labels is to first aggregate them into one and apply standard training methods. The literature has also studied extensively on effective aggregation approaches. This paper revisits this choice and aims to provide an answer to the question of whether one should aggregate separate noisy labels into single ones or use them separately as given. We theoretically analyze the performance of both approaches under the empirical risk minimization framework for a number of popular loss functions, including the ones designed specifically for the problem of learning with noisy labels. Our theorems conclude that label separation is preferred over label aggregation when the noise rates are high, or the number of labelers/annotations is insufficient. Extensive empirical results validate our conclusions.

==> src/backup.tex <==


% \subsection{Additional Experiment Results on Two more UCI Datasets}

% \begin{table*}[!ht]
% \centering{\scalebox{0.60}{
% \begin{tabular}{ccccccc||ccccccc}
% \hline
% \multicolumn{7}{c}{\emph{UCI-pop failuers (symmetric) CE}}& \multicolumn{7}{c}{\emph{UCI-forest fire (symmetric) CE}}  \\
% \hline
%  $\epsilon=0.2$&  $K=3$ & $K=5$ & $K=9$ & $K=15$ & $K=25$ & $K=49$ &$\epsilon=0.2$&  $K=3$ & $K=5$ & $K=9$ & $K=15$ & $K=25$ & $K=49$\\ \hline\hline
%  MV & \better{93.06}  & 93.06 & 93.06 & 93.06 & 93.06 & 93.06  & MV & 92.86 & 92.86 & 91.84 & 91.84 & \better{91.84} & 91.84\\
% EM  &\better{93.06}  & 93.06 & 93.06 & 93.06 & 93.06 & 93.06  &  EM  & 92.86 & 92.86 & 91.84 & 91.84 & \better{91.84} & 91.84 \\
% Sep & \good{93.06}  & \good{93.52} & \good{93.98}  & \good{94.91} & \good{95.83}  & \good{96.30}  & Sep  & \good{93.88} & \good{93.88} & \good{95.92} & \good{94.90} & \good{91.84} & \good{93.88} \\
%  \hline
%  \hline
%  $\epsilon=0.4$&  $K=3$ & $K=5$ & $K=9$ & $K=15$ & $K=25$ & $K=49$ & $\epsilon=0.4$&  $K=3$ & $K=5$ & $K=9$ & $K=15$ & $K=25$ & $K=49$ \\ \hline\hline
%   MV  & \better{93.06} & 93.06 & 93.06& 93.06 & 93.06 & 93.06 & MV  & \better{81.63}  & \better{81.63}  & \better{90.82} & \better{91.84} & \better{91.84} &  91.84  \\
% EM & \better{93.06} & 93.06 & 93.06 & 93.52 & 93.06 & 93.52  &  EM   & 58.16  & 77.55  & \better{90.82} & 88.78 & 91.84  & 91.84 \\
% Sep & \good{93.06} &\good{93.52}& \good{93.98} & \good{94.91} & \good{95.37} & \good{95.37} & Sep & 79.59  & 79.59  & 87.76 & 87.76 &  90.82  & \good{92.86}\\
%  \hline\hline
% \multicolumn{7}{c}{\emph{UCI-pop failuers (symmetric) BW}}& \multicolumn{7}{c}{\emph{UCI-forest fire (symmetric) BW}}  \\
% \hline
%  $\epsilon=0.2$&  $K=3$ & $K=5$ & $K=9$ & $K=15$ & $K=25$ & $K=49$ &$\epsilon=0.2$&  $K=3$ & $K=5$ & $K=9$ & $K=15$ & $K=25$ & $K=49$\\ \hline\hline
%  MV  & \better{93.06} & 93.06&  93.06  & 93.06 & 93.06 & 93.06   & MV    & \better{91.84} & \better{92.86}& 91.84 & 91.84 & \better{91.84}& 92.86 \\
% EM & \better{93.06} & 93.06 & 93.06 & 93.06 & 93.06 & 93.06   &  EM   & \better{91.84} & \better{92.86} & 91.84 & 91.84 & \better{91.84} & 92.86  \\
% Sep & \good{93.06}  & \good{93.52} & \good{93.98}  & \good{95.37} & \good{95.83}  & \good{95.83}  & Sep  & 88.78 & 90.82 & \good{92.86} & \good{93.88} & \good{91.84} & \good{94.90}  \\
%  \hline
%  \hline
%  $\epsilon=0.4$&  $K=3$ & $K=5$ & $K=9$ & $K=15$ & $K=25$ & $K=49$ & $\epsilon=0.4$&  $K=3$ & $K=5$ & $K=9$ & $K=15$ & $K=25$ & $K=49$ \\ \hline\hline
%   MV  & 92.13 & 90.59& 90.59 & 90.59 & 92.91 & 93.06 & MV  & \better{84.69}  & \better{86.73}  & \better{89.80} & \better{91.84} & \better{91.84} & \better{92.86}  \\
% EM & \better{93.06} & 89.35 & \better{93.06} & \better{91.20} & 93.06 & 93.06 &  EM & 73.47 & 75.51 & 88.78 & \better{91.84}& \better{91.84}  & 91.84  \\
% Sep & \good{93.06} & \good{93.06} & \good{93.06}  & \good{91.20}  & \good{93.98} & \good{94.91} & Sep  & \good{84.69} & 84.69  & 86.73  & 87.76 & 86.73 & 90.82\\
%  \hline\hline
% \multicolumn{7}{c}{\emph{UCI-pop failuers (symmetric) Peer Loss}}& \multicolumn{7}{c}{\emph{UCI-forest fire (symmetric) Peer Loss}}  \\
% \hline
%  $\epsilon=0.2$&  $K=3$ & $K=5$ & $K=9$ & $K=15$ & $K=25$ & $K=49$ &$\epsilon=0.2$&  $K=3$ & $K=5$ & $K=9$ & $K=15$ & $K=25$ & $K=49$\\ \hline\hline
%  MV  & \better{93.06} & \better{93.52} & 94.91 & \better{94.44}  & 94.44  & 94.44  & MV  & \better{92.86} & \better{92.86} & 92.86 & 92.86 & \better{92.86} & \better{94.90}      \\
% EM  & \better{93.06} & \better{93.06} & \better{94.44}  & \better{94.44} & 94.44  & 94.44   &  EM  & \better{92.86} & \better{92.86} & 92.86 & 92.86 & \better{92.86} & \better{94.90}   \\
% Sep & \good{93.06} & 92.59  & 93.98  & \good{94.44} & \good{95.83}  & \good{97.22}    & Sep   & 88.78 & 89.80 & \good{93.88} & \good{93.88} & \good{92.86} & \good{94.90} \\
%  \hline
%  \hline
%  $\epsilon=0.4$&  $K=3$ & $K=5$ & $K=9$ & $K=15$ & $K=25$ & $K=49$ & $\epsilon=0.4$&  $K=3$ & $K=5$ & $K=9$ & $K=15$ & $K=25$ & $K=49$ \\ \hline\hline
%   MV & \better{93.06} & \better{93.52} & \better{93.52} & \better{93.98}  & 94.91 & 93.52& MV & 78.57  & 78.57  & \better{89.80} & \better{91.84} & 89.80 & 91.84     \\
% EM & \better{93.06} & 93.06 & 93.06 & \better{93.98} & 93.06 & 93.52 &  EM   & 59.18  & 73.47 & 88.78 & 89.80 & 89.80 & 91.84  \\
% Sep  & 88.89 & 92.59 & 92.59  & \good{93.98}  & \good{95.83}  & \good{95.37} & Sep   & \good{83.67}  & \good{80.61}  & 85.71  & 88.78 & \good{91.84} & \good{92.86}  \\
% \hline
% \end{tabular}}}
% % \vspace{5pt}
% \caption{The performances of CE/BW/PeerLoss trained on two additional UCI datasets (Climate Model Simulation Crashes and Algerian Forest Fires datasets), with aggregated labels (majority vote, EM inference), and separated labels. ($K$ is the number of labels per training image) 
% }
% \label{Tab:uci_s_o_ce}
% \end{table*}

\begin{table*}[!b]
\centering{\scalebox{0.7}{
\begin{tabular}{ccccccc||ccccccc}
\hline
\multicolumn{7}{c}{\emph{UCI-StatLog (symmetric) CE}}& \multicolumn{7}{c}{\emph{UCI-Optical (symmetric) CE}}  \\
\hline
 $\epsilon=0.2$&  $K=3$ & $K=5$ & $K=9$ & $K=15$ & $K=25$ & $K=49$ &$\epsilon=0.2$&  $K=3$ & $K=5$ & $K=9$ & $K=15$ & $K=25$ & $K=49$\\ \hline\hline
 MV  & 87.94 & 88.88 & 88.69 & 88.69 & 88.69 & 88.69   & MV   & 95.27  & 96.73  & 95.41  & 96.73  & 96.73  & 96.66   \\
EM   & 87.63 & 87.94 & 88.63 & 88.69 & 88.69 & 88.69  & EM & 95.34  & 95.69 & 96.04& 96.73  & 96.73  & 96.73   \\
Sep   & \good{}89.25 & \good{}90.56 & \good{}91.19 & \good{}91.13 & \good{}91.50 & \good{}91.25  & Sep  & \good{}97.08 & \good{}97.57 & \good{}97.98  & 98.33  & \good{}98.26  & \good{}98.61    \\
 \hline
 \hline
 $\epsilon=0.4$&  $K=3$ & $K=5$ & $K=9$ & $K=15$ & $K=25$ & $K=49$ & $\epsilon=0.4$&  $K=3$ & $K=5$ & $K=9$ & $K=15$ & $K=25$ & $K=49$ \\ \hline\hline
 MV  & 87.00 & 87.50 & 88.25 & 88.63 & 88.75 & 88.69  & MV & 92.35  & 96.04 & 96.11 & 96.18 & 96.73  & 96.73  \\
EM   & 87.50 & 87.38& 87.75 & 88.94 & 88.81  & 88.69  & EM  & 93.25 & 94.78 & 95.68  & 96.03  & 96.73  & 96.73  \\
Sep   & \good{}87.75 & \good{}89.31  & \good{}90.38& \good{}91.19 & \good{}91.19 & \good{}91.00  & Sep  & \good{}96.59 & \good{}96.80 &\good{} 97.44 &\good{} 97.64 &\good{} 98.26  & \good{}98.05  \\
 \hline
 \hline
 $\epsilon=0.6$&  $K=3$ & $K=5$ & $K=9$ & $K=15$ & $K=25$ & $K=49$ & $\epsilon=0.6$&  $K=3$ & $K=5$ & $K=9$ & $K=15$ & $K=25$ & $K=49$ \\ \hline\hline
 MV   & 80.75 & 85.00 & 86.75 & 87.25 & 87.75 & 88.62    & MV   & 83.31  & 91.51  & 95.34  & 95.41  & 93.11  & 97.14 \\
EM   & 85.06  & 84.37  & 86.68  & 87.00 & 87.81  & 88.93    & EM  & 88.31  & 92.35  & 93.81  & 95.13  & 96.31  & 95.96 \\
Sep  & \good{}87.18  & \good{}87.31  & \good{}88.12  & \good{}89.81  &\good{} 90.81  & \good{}90.93    & Sep   & \good{}94.43  & \good{}95.54 & \good{}96.52  &\good{} 97.35  & \good{}97.63  & \good{}97.98  \\
%  \hline
%  \hline
%  $\epsilon=0.8$&  $K=3$ & $K=5$ & $K=9$ & $K=15$ & $K=25$ & $K=49$ & $\epsilon=0.8$&  $K=3$ & $K=5$ & $K=9$ & $K=15$ & $K=25$ & $K=49$ \\ \hline\hline
%  MV  & 32.43 & 33.25 & 47.87 & 64.87  & 78.43  & 81.31  & MV   & 34.90  & 52.85  & 76.84  & 84.14  & 91.72  & 93.46   \\
% EM  & 59.25 & 53.68 & 75.00 & \bad{} 78.93  & \bad{} 79.43  &\bad{} 82.93   & EM   & 55.42  & 44.15  & 68.56  & 80.73  & 85.95  & 90.61   \\
% Sep  & \good{}72.06 & \good{}74.68  & \good{}76.00 & 77.37  & 74.93  & 81.12    & Sep  & \good{}84.70  &\good{} 86.36  &\good{} 90.68  & \good{}92.48  &\good{} 93.88  & \good{}95.75  \\
 \hline\hline
\multicolumn{7}{c}{\emph{UCI-StatLog (symmetric) BW }}& \multicolumn{7}{c}{\emph{UCI-Optical (symmetric) BW}}  \\
\hline
 $\epsilon=0.2$&  $K=3$ & $K=5$ & $K=9$ & $K=15$ & $K=25$ & $K=49$ &$\epsilon=0.2$&  $K=3$ & $K=5$ & $K=9$ & $K=15$ & $K=25$ & $K=49$\\ \hline\hline
 MV  & 89.75 & 90.06  & 89.87  & 89.87  & 89.87 & 89.87   & MV   & 94.43  & 95.41 & 95.61  & 96.94  & 96.94  & 96.94  \\
EM & 89.68 & 89.87  & 89.75 & 89.87  & 89.87  & 89.87    & EM  & 94.43  & 95.82  & 95.68  & 96.94  & 96.94  & 96.94   \\
Sep  & \good{}89.87  & \good{}91.18 & \good{}92.00 &\good{} 91.43  & \good{}91.37  & \good{}91.06    & Sep   & \good{}96.87  & \good{}97.21  & \good{}97.63  & \good{}97.77  & \good{}98.05 & \good{}97.63  \\
 \hline
 \hline
 $\epsilon=0.4$&  $K=3$ & $K=5$ & $K=9$ & $K=15$ & $K=25$ & $K=49$ & $\epsilon=0.4$&  $K=3$ & $K=5$ & $K=9$ & $K=15$ & $K=25$ & $K=49$ \\ \hline\hline
 MV  & 87.62  & 88.25 & 89.75 & 89.62  & 89.87  & 89.87   & MV  & 90.19  & 94.29  & 94.64  & 96.80  & 96.94  & 96.94 \\
EM  & 87.93  & 88.31 & 89.56   & 89.81  & 89.75 & 89.87   & EM   & 93.53 & 95.41 & 96.38 & 95.89  & 96.94  & 96.94    \\
Sep & \good{}89.62  &\good{} 89.87 & \good{}90.18  & \good{}91.00 & \good{}91.06  & \good{}91.37   & Sep  & \good{}95.54  & \good{}96.59  & \good{}96.66  & \good{}97.28  & \good{}97.77  & \good{}97.77 \\
 \hline
 \hline
 $\epsilon=0.6$&  $K=3$ & $K=5$ & $K=9$ & $K=15$ & $K=25$ & $K=49$ & $\epsilon=0.6$&  $K=3$ & $K=5$ & $K=9$ & $K=15$ & $K=25$ & $K=49$ \\ \hline\hline
 MV  & 82.12  & 87.31 & 87.00 & 88.50 & 89.50 & 89.81    & MV   & 82.54  & 88.10  & 92.97  & 95.75  & 93.67  & 96.52   \\
EM & \bad{}86.68  & 86.50 & 87.31  & 88.25 & 89.12 & 89.81  & EM  & 80.52  & 90.54 & 93.11  & 95.06  & 96.10  & 95.82   \\
Sep  & 86.18  &\good{} 87.62  & \good{}88.31  & \good{}89.62  & \good{}90.93  & \good{}90.75  & Sep  & \good{}91.72  & \good{}93.39  & \good{}93.46  & \good{}96.38  & \good{}96.66  & \good{}97.21  \\
%  \hline
%  \hline
%  $\epsilon=0.8$&  $K=3$ & $K=5$ & $K=9$ & $K=15$ & $K=25$ & $K=49$ & $\epsilon=0.8$&  $K=3$ & $K=5$ & $K=9$ & $K=15$ & $K=25$ & $K=49$ \\ \hline\hline
%  MV   & 23.68 & 45.06 & 71.00 & 74.68  & 76.56  & 78.56   & MV & 51.46  & 51.11  & 74.33  & 78.23  & 87.62  & 93.39    \\
% EM  & 69.37  & 50.06  & 60.25 & 81.12  & 68.75 & 78.50  & EM  & 53.61  & 34.97  & 63.90 & 60.36 & 83.10  & 90.68    \\
% Sep  & 64.75 &   & 58.50 & 54.75 & 76.19 & 25.38    & Sep   & 62.58  & 65.57 & 76.77  & 85.39  & 83.65  & 91.72    \\
 \hline
\hline
\multicolumn{7}{c}{\emph{UCI-StatLog (symmetric) PeerLoss }}& \multicolumn{7}{c}{\emph{UCI-Optical (symmetric) PeerLoss}}  \\
\hline
 $\epsilon=0.2$&  $K=3$ & $K=5$ & $K=9$ & $K=15$ & $K=25$ & $K=49$ &$\epsilon=0.2$&  $K=3$ & $K=5$ & $K=9$ & $K=15$ & $K=25$ & $K=49$\\ \hline\hline
 MV   & 90.25 & 90.06 & 90.56  & 90.56  & 90.56  & 90.56   & MV  & 94.71  & 96.03  & 96.38  & 96.52  & 96.52  & 96.38   \\
EM  & 89.87  & 90.06  & 90.56  & 90.56  & 90.56  & 90.56    & EM  & 94.43  & 96.17  & 96.52  & 96.52  & 96.52  & 96.52   \\
Sep & \good{}90.36  & \good{}91.12 & \good{}91.68  &\good{} 91.43  & \good{}91.68  &\good{} 91.43  & Sep   & \good{}97.07  & \good{}97.35  & \good{}97.70 & \good{}98.12  &\good{} 98.05  & \good{}98.12  \\
 \hline
 \hline
 $\epsilon=0.4$&  $K=3$ & $K=5$ & $K=9$ & $K=15$ & $K=25$ & $K=49$ & $\epsilon=0.4$&  $K=3$ & $K=5$ & $K=9$ & $K=15$ & $K=25$ & $K=49$ \\ \hline\hline
 MV   & 87.93  & 89.06  & 90.18 & 90.43  & 90.68  & 90.56   & MV  & 91.86  & 94.57  & 95.54  & 96.87  & 96.52  & 96.52   \\
EM  & 88.00 & 88.93  & 90.12  & 90.37  & 90.56  & 90.56   & EM  & 91.86 & 93.94  & 95.96  & 96.87  & 96.52  & 96.52 \\
Sep   & \good{}89.18  & \good{}90.25 & \good{}90.37  &\good{} 91.43  & \good{}91.68  &\good{} 91.87     & Sep   & \good{}96.66  & \good{}96.73  & \good{}96.94  &\good{} 97.63  & \good{}98.05  &\good{}98.19  \\
 \hline
 \hline
 $\epsilon=0.6$&  $K=3$ & $K=5$ & $K=9$ & $K=15$ & $K=25$ & $K=49$ & $\epsilon=0.6$&  $K=3$ & $K=5$ & $K=9$ & $K=15$ & $K=25$ & $K=49$ \\ \hline\hline
 MV  & 78.68  & 86.68  & 87.31  & 88.81  & 89.75 & 90.56   & MV  & 76.77 & 87.34  & 94.71  & 95.61  & 93.88  & 96.38 \\
EM  & 86.25 & 86.68  & 88.00 & 88.75 & 89.12  & 90.31   & EM  & 86.92 & 89.98  & 93.11 & 96.10  & 95.82  & 96.10 \\
Sep  & \good{}87.50 & \good{}88.25 & \good{}88.93  & \good{}90.18  & \good{}91.31  & \good{}91.31    & Sep   & \good{}93.32  & \good{}95.54  & \good{}96.10  & \good{}96.73 &\good{} 97.77 & \good{}97.91  \\
\hline
\hline
\multicolumn{7}{c}{\emph{UCI-pop failuers (symmetric) CE}}& \multicolumn{7}{c}{\emph{UCI-forest fire (symmetric) CE}}  \\
\hline
 $\epsilon=0.2$&  $K=3$ & $K=5$ & $K=9$ & $K=15$ & $K=25$ & $K=49$ &$\epsilon=0.2$&  $K=3$ & $K=5$ & $K=9$ & $K=15$ & $K=25$ & $K=49$\\ \hline\hline
 MV & \better{93.06}  & 93.06 & 93.06 & 93.06 & 93.06 & 93.06  & MV & 92.86 & 92.86 & 91.84 & 91.84 & \better{91.84} & 91.84\\
EM  &\better{93.06}  & 93.06 & 93.06 & 93.06 & 93.06 & 93.06  &  EM  & 92.86 & 92.86 & 91.84 & 91.84 & \better{91.84} & 91.84 \\
Sep & \good{93.06}  & \good{93.52} & \good{93.98}  & \good{94.91} & \good{95.83}  & \good{96.30}  & Sep  & \good{93.88} & \good{93.88} & \good{95.92} & \good{94.90} & \good{91.84} & \good{93.88} \\
 \hline
 \hline
 $\epsilon=0.4$&  $K=3$ & $K=5$ & $K=9$ & $K=15$ & $K=25$ & $K=49$ & $\epsilon=0.4$&  $K=3$ & $K=5$ & $K=9$ & $K=15$ & $K=25$ & $K=49$ \\ \hline\hline
  MV  & \better{93.06} & 93.06 & 93.06& 93.06 & 93.06 & 93.06 & MV  & \better{81.63}  & \better{81.63}  & \better{90.82} & \better{91.84} & \better{91.84} &  91.84  \\
EM & \better{93.06} & 93.06 & 93.06 & 93.52 & 93.06 & 93.52  &  EM   & 58.16  & 77.55  & \better{90.82} & 88.78 & 91.84  & 91.84 \\
Sep & \good{93.06} &\good{93.52}& \good{93.98} & \good{94.91} & \good{95.37} & \good{95.37} & Sep & 79.59  & 79.59  & 87.76 & 87.76 &  90.82  & \good{92.86}\\
 \hline\hline
\multicolumn{7}{c}{\emph{UCI-pop failuers (symmetric) BW}}& \multicolumn{7}{c}{\emph{UCI-forest fire (symmetric) BW}}  \\
\hline
 $\epsilon=0.2$&  $K=3$ & $K=5$ & $K=9$ & $K=15$ & $K=25$ & $K=49$ &$\epsilon=0.2$&  $K=3$ & $K=5$ & $K=9$ & $K=15$ & $K=25$ & $K=49$\\ \hline\hline
 MV  & \better{93.06} & 93.06&  93.06  & 93.06 & 93.06 & 93.06   & MV    & \better{91.84} & \better{92.86}& 91.84 & 91.84 & \better{91.84}& 92.86 \\
EM & \better{93.06} & 93.06 & 93.06 & 93.06 & 93.06 & 93.06   &  EM   & \better{91.84} & \better{92.86} & 91.84 & 91.84 & \better{91.84} & 92.86  \\
Sep & \good{93.06}  & \good{93.52} & \good{93.98}  & \good{95.37} & \good{95.83}  & \good{95.83}  & Sep  & 88.78 & 90.82 & \good{92.86} & \good{93.88} & \good{91.84} & \good{94.90}  \\
 \hline
 \hline
 $\epsilon=0.4$&  $K=3$ & $K=5$ & $K=9$ & $K=15$ & $K=25$ & $K=49$ & $\epsilon=0.4$&  $K=3$ & $K=5$ & $K=9$ & $K=15$ & $K=25$ & $K=49$ \\ \hline\hline
  MV  & 92.13 & 90.59& 90.59 & 90.59 & 92.91 & 93.06 & MV  & \better{84.69}  & \better{86.73}  & \better{89.80} & \better{91.84} & \better{91.84} & \better{92.86}  \\
EM & \better{93.06} & 89.35 & \better{93.06} & \better{91.20} & 93.06 & 93.06 &  EM & 73.47 & 75.51 & 88.78 & \better{91.84}& \better{91.84}  & 91.84  \\
Sep & \good{93.06} & \good{93.06} & \good{93.06}  & \good{91.20}  & \good{93.98} & \good{94.91} & Sep  & \good{84.69} & 84.69  & 86.73  & 87.76 & 86.73 & 90.82\\
 \hline\hline
\multicolumn{7}{c}{\emph{UCI-pop failuers (symmetric) Peer Loss}}& \multicolumn{7}{c}{\emph{UCI-forest fire (symmetric) Peer Loss}}  \\
\hline
 $\epsilon=0.2$&  $K=3$ & $K=5$ & $K=9$ & $K=15$ & $K=25$ & $K=49$ &$\epsilon=0.2$&  $K=3$ & $K=5$ & $K=9$ & $K=15$ & $K=25$ & $K=49$\\ \hline\hline
 MV  & \better{93.06} & \better{93.52} & 94.91 & \better{94.44}  & 94.44  & 94.44  & MV  & \better{92.86} & \better{92.86} & 92.86 & 92.86 & \better{92.86} & \better{94.90}      \\
EM  & \better{93.06} & \better{93.06} & \better{94.44}  & \better{94.44} & 94.44  & 94.44   &  EM  & \better{92.86} & \better{92.86} & 92.86 & 92.86 & \better{92.86} & \better{94.90}   \\
Sep & \good{93.06} & 92.59  & 93.98  & \good{94.44} & \good{95.83}  & \good{97.22}    & Sep   & 88.78 & 89.80 & \good{93.88} & \good{93.88} & \good{92.86} & \good{94.90} \\
 \hline
 \hline
 $\epsilon=0.4$&  $K=3$ & $K=5$ & $K=9$ & $K=15$ & $K=25$ & $K=49$ & $\epsilon=0.4$&  $K=3$ & $K=5$ & $K=9$ & $K=15$ & $K=25$ & $K=49$ \\ \hline\hline
  MV & \better{93.06} & \better{93.52} & \better{93.52} & \better{93.98}  & 94.91 & 93.52& MV & 78.57  & 78.57  & \better{89.80} & \better{91.84} & 89.80 & 91.84     \\
EM & \better{93.06} & 93.06 & 93.06 & \better{93.98} & 93.06 & 93.52 &  EM   & 59.18  & 73.47 & 88.78 & 89.80 & 89.80 & 91.84  \\
Sep  & 88.89 & 92.59 & 92.59  & \good{93.98}  & \good{95.83}  & \good{95.37} & Sep   & \good{83.67}  & \good{80.61}  & 85.71  & 88.78 & \good{91.84} & \good{92.86}  \\
\hline
\end{tabular}}}
% \vspace{5pt}
\caption{The performances of CE/BW/PeerLoss trained on 4 UCI datasets (StatLog, Optical, Pop-Failures, and Forest Fair datasets), with aggregated labels (majority vote, EM inference), and separated labels. ($K$ is the number of labels per training image) 
}
\label{Tab:uci_s_o_ce}
\end{table*}



